Waypoint-Based Reinforcement Learning for Robot Manipulation Tasks

Robot arms should be able to learn new tasks. One framework here is reinforcement learning, where the robot is given a reward function that encodes the task, and the robot autonomously learns actions to maximize its reward. Existing approaches to reinforcement learning often frame this problem as a Markov decision process, and learn a policy (or a hierarchy of policies) to complete the task. These policies reason over hundreds of fine-grained actions that the robot arm needs to take: e.g., moving slightly to the right or rotating the end-effector a few degrees. But the manipulation tasks that we want robots to perform can often be broken down into a small number of high-level motions: e.g., reaching an object or turning a handle. In this paper we therefore propose a waypoint-based approach for model-free reinforcement learning. Instead of learning a low-level policy, the robot now learns a trajectory of waypoints, and then interpolates between those waypoints using existing controllers. Our key novelty is framing this waypoint-based setting as a sequence of multi-armed bandits: each bandit problem corresponds to one waypoint along the robot's motion. We theoretically show that an ideal solution to this reformulation has lower regret bounds than standard frameworks. We also introduce an approximate posterior sampling solution that builds the robot's motion one waypoint at a time. Results across benchmark simulations and two real-world experiments suggest that this proposed approach learns new tasks more quickly than state-of-the-art baselines. See videos here: https://youtu.be/MMEd-lYfq4Y

==> archive.tex <==
\section{Method}


% what follows is the result of our hypothesis (splitting into waypoints)

\p{Trajectory} Under our proposed approach we control the robot arm to follow a trajectory.
Let $s_\mathcal{R} \in \mathcal{S}_\mathcal{R} \subseteq \mathcal{S}$ be the state of the robot arm (e.g., the pose of the robot's end-effector).
We define the robot's reference trajectory as: $\xi_\mathcal{R} = \{s_\mathcal{R}^0, \ldots, s_\mathcal{R}^T\}$, where each robot state $s_\mathcal{R}$ is a \textit{waypoint}, and $T$ is the number of waypoints.
We constrain $T < H$, so that the number of waypoints is less than the total number of timesteps.

\p{Controller} We assume access to a low-level robot controller that takes actions $a$ to move the robot arm along trajectory $\xi_\mathcal{R}$.
There are a variety of robot controllers for tracking reference trajectories \cite{}, and in our experiments we use impedance control \cite{}.
In practice, this controller causes the robot arm to interpolate between the waypoints while remaining compliant if the robot comes into contact with objects in the environment.

As the robot moves to track its trajectory $\xi_\mathcal{R}$, the robot's actions $a$ cause the system to transition to new world states $s$.
Let $\xi = \{s^0, \ldots, s^H \}$ be the trajectory of world states visited during a single interaction.
Importantly, this trajectory of world states is a function of the robot's trajectory:
\begin{equation}
    \xi \sim f(\xi_\mathcal{R})
\end{equation}

% % problem --- find the trajectory that will maximize the expected cumulative reward
% % need to define expected cumulative reward - reward over xi


% There is an unknown function $g(\xi_\mathcal{R}) \rightarrow \xi$ that maps the trajectory the robot is executing $\xi_\mathcal{R}$ to a sequence of world states $\xi$.

% This unknown function $g$ is determined connected to the world dynamics $f$ and the controller used to execute trajectory $\xi_\mathcal{R}$.



\p{Trajectory} Let $\xi_\mathcal{R} = \{s_\mathcal{R}^1, \ldots, s_\mathcal{R}^T\}$ be a robot trajectory with $T$ waypoints, where $T \leq H$. This trajectory could be in the robot's end-effector space or joint space. We assume access to a controller that makes the robot follow this trajectory (e.g., an impedance controller). In practice, the controller causes the robot to take actions that interpolate between the waypoints. Let $\xi = \{s^1, \ldots s^H\}$ be the sequence of world states that the robot visits throughout one episode of the MDP $\mathcal{M}$. There is an unknown function $g(\xi_\mathcal{R}) \rightarrow \xi$ that maps the trajectory the robot is executing $\xi_\mathcal{R}$ to a sequence of world states $\xi$. This unknown function $g$ is determined connected to the world dynamics $f$ and the controller used to execute trajectory $\xi_\mathcal{R}$.

\p{MAB} We write this problem as a continuous multi-armed bandit. The continuous space of arms is $\xi_\mathcal{R} \in \Xi_\mathcal{R} \subseteq \mathbb{R}^{T \times n}$, where $n$ is the dimension of the robot's state space. Once an arm is selected, the robot plays that arm by executing trajectory $\xi_\mathcal{R}$ and observing the outcome $\xi = g(\xi_\mathcal{R})$. The robot gets total reward $R(g(\xi_\mathcal{R})) = R(\xi) = \sum_{t=1}^H r(s^t)$. Define $R^*$ as the expected reward for the best possible arm. Our objective is to minimize the robot's regret across $K$ interactions:
\begin{equation}
    REG = \sum_{k=1}^K \big(R^* - R(g(\xi_\mathcal{R}^k)\big)
\end{equation}

% note that therea re a few approaches, this is a bit more general than one specific solution
% Under this novel formulation, all policy optimization algorithms can be used for option
% learning and master policy learning off the shelf and the learning remains intra-option. 

\p{Approach} Under our formulation the robot is uncertain about $g$ (e.g., how a given trajectory will map to changes in world state). Instead of directly trying to learn $g$, we instead learn $R(g( \cdot ))$. In other words, we attempt to learn the mapping from robot trajectories to cumulative rewards:
\begin{equation}
    R_\theta(\xi_\mathcal{R}) \rightarrow \mathbb{R}
\end{equation}
where $R_\theta$ is a neural network with parameters $\theta$. Our rational here is that we only care about $g$ in so far as it affects the reward function --- i.e., we only care about $g$ so we can evaluate $R(g(\cdot))$ --- and so it is more efficient to learn the reward function $R_\theta(\cdot) = R(g(\cdot))$. This is also analogous to multi-armed bandit settings, where we seek to learn the expected rewards associated with each arm.

\p{Algorithm} Our proposed approach is an extension of Ensemble Sampling \cite{lu2017ensemble}, which seeks to approximate Thompson Sampling (TS) and can be applied to continuous multi-armed bandits. TS is a heuristic approach to minimize regret on multi-armed bandits with strong theoretical support over the years. The core idea is to maintain an ensemble of reward models $R_{\theta_i}$. At each episode a reward model from this ensemble is randomly selected, and the robot uses nonlinear constrained optimization to find the trajectory $\xi_\mathcal{R}$ that is optimal with respect to this reward function. The robot then executes the trajectory $\xi_\mathcal{R}$ and we observe the resulting reward $R = R(g(\xi_\mathcal{R}))$. This builds a dataset of $(\xi_\mathcal{R}, R)$ pairs that we leverage to train the reward models. See Algorithm~\ref{alg:ensemble}.

\begin{algorithm}[t] 
\caption{Version 1}
\label{alg:ensemble}
\begin{algorithmic}[1] 
\State Initialize $N$ reward models with weights $\theta_1, \ldots, \theta_N$
\For {each interaction}
    \State Sample a random index $i \sim \text{uniform}(1, N)$
    \State $\xi_\mathcal{R} \gets \text{arg}\max_{\Xi_\mathcal{R}} R_{\theta_i}(\xi)$ \Comment Trajectory Optimization
    \State Rollout $\xi_\mathcal{R}$ in MDP $\mathcal{M}$ \Comment Robot Control
    \State Observe total reward $R$ and record $\mathcal{D} \gets (\xi_\mathcal{R}, R)$    
    \For {each reward model $i$}
        \State Sample batch $\mathcal{B}$ from $\mathcal{D}$
        \State $\mathcal{L}_i \gets \sum_{(\xi_\mathcal{R}, R)\in \mathcal{B}} \| R_{\theta_i}(\xi_\mathcal{R}) - R \| $
        \State Update $\theta_i$ to minimize $\mathcal{L}_i$
    \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}

\p{Implementation Details} When using nonlinear optimization to find the best trajectory in Algorithm~\ref{alg:ensemble} (Line 4), the search can get stuck in local minima. We recommend (a) seeding the search with the best performing trajectory observed so far, and (b) performing the optimization multiple times in parallel, and then selecting the trajectory with the best overall reward.

\p{Loss Function} In Algorithm~\ref{alg:ensemble} we train the reward models using the MSE loss. Alternatively, we could train the reward models to rank the trajectories correctly using a cross-entropy loss. This approach could help the robot extrapolate regions of the workspace where higher rewards occur. We have not implemented or tested this approach, and I do not anticipate any major differences in performance.

\subsection{Theoretical analysis: Why is this a good idea?}

% In development.

Does reducing the dimensionality of the space help?
Our key assumption is that we are dealing with settings where the robot's optimal behavior is captured by a finite, small number of waypoints. But we could instead apply our same approach where there are H waypoints. Is there any advantage to looking for a trajectory with fewer waypoints?
We look specifically at MABs. 
--- We are currently trying to find the lower bound for MABs in continuous (maybe Lipschitz) spaces.
It seems like it is polynomial in d and sublinear in K if the reward space is convex, and some other restrictions are met. But generally the space explodes.
for contextual bandits (which appear related), the lower bound is something like O(sqrt(dK)), where K is the number of interactions and d is the dimension of the space.
So lower dimensions = better
But if we go too low, then we will miss out on part of the motion; in this case, our long-term regret becomes something more like O(K)
Simulation results with our approach support this: intuitively, we get better performance faster by reducing the dimension, but if we reduce it too much we will eventually be beaten out by approaches that do not use waypoints.
Current result: decreasing dimension to waypoints has benefits under MAB formulation.
So the benefit is fewer decisions (accelerating search), the downside is lack of resolution (reducing the maximum possible reward).
So we can prove that --- under our framework --- waypoints is better than a complete trajectory, provided the task only needs these waypoints
Desired result: extend to comparison with RL-like algorithms



% idea: get lower bounds on performance for RL and MAB. Then see where the crossover is between the two.

% bandit: no matter what algorithm we choose, our best-case regret (lower bound on regret) is:
\begin{equation}
    O(\sqrt{AK})
\end{equation}
% https://arxiv.org/pdf/1608.02732.pdf
% ideally we want to design algorithms with upper bounds near these lower bounds

% episodic MDP: lower bound appears to be:
\begin{equation}
    O(\sqrt{H^2SAK})
\end{equation}
% http://proceedings.mlr.press/v132/domingues21a/domingues21a.pdf
% https://proceedings.neurips.cc/paper_files/paper/2008/file/e4a6222cdb5b34375400904f03d8e6a5-Paper.pdf
% where H is length of episode and K is the number of episodes
% http://proceedings.mlr.press/v70/osband17a/osband17a.pdf
% it looks like TS for RL is reasonably close to the bound, with this paper acheiving O(H sqrt(HSAK))
% https://arxiv.org/pdf/1608.02732.pdf
% this paper suggests that the bound above is unimprovable, where D=H and T = HK

% under our proposed approach we are writing the MDP as a MAB with S_R^T arms, where S_R is the dimension of the robot's state and T is the number of waypoints
% So the fundamental tradeoff is the comparison of:
\begin{equation}
    \mathcal{S}_\mathcal{R}^T \leq H^2 \mathcal{S}\mathcal{A}
\end{equation}
% If we can show this holds, then our approach appears theoretically advantageous, and this advantage is not tied to a specific algorithm but rather to a problem structure
% intuitively, this happens when the ratio of T / H is very small: if we only need a couple waypoints, but H is very long, then H^2 is worse than S_R^T. I do see H and T as the dominant terms, but it should be reflected that this could also break as S_R expands

% would be good to prove this in a finite state / action MDP
